MaskINT: Video Editing via Interpolative Non-autoregressive Masked Transformers

Recent advances in generative AI have significantly enhanced image and video editing, particularly in the context of text prompt control. State-of-the-art approaches predominantly rely on diffusion models to accomplish these tasks. However, the computational demands of diffusion-based methods are substantial, often necessitating large-scale paired datasets for training, and therefore challenging the deployment in real applications. To address these issues, this paper breaks down the text-based video editing task into two stages. First, we leverage an pre-trained text-to-image diffusion model to simultaneously edit few keyframes in an zero-shot way. Second, we introduce an efficient model called MaskINT, which is built on non-autoregressive masked generative transformers and specializes in frame interpolation between the edited keyframes, using the structural guidance from intermediate frames. Experimental results suggest that our MaskINT achieves comparable performance with diffusion-based methodologies, while significantly improve the inference time. This research offers a practical solution for text-based video editing and showcases the potential of non-autoregressive masked generative transformers in this domain.

==> sec2/0_abstract.tex <==
\begin{abstract}
Recent advances in generative AI have significantly enhanced image and video editing, particularly in the context of text prompt control. State-of-the-art approaches predominantly rely on diffusion models to accomplish these tasks. However, the computational demands of diffusion-based methods are substantial, often necessitating large-scale paired datasets for training, and therefore challenging the deployment in practical applications.
This study addresses this challenge by breaking down the text-based video editing process into two stages. In the first stage, we leverage an existing text-to-image diffusion model to simultaneously edit a few selected key frames without any additional fine-tuning. In the second stage, we introduce an efficient model called MaskINT, which is built on non-autoregressive masked generative transformers. MaskINT specializes in frame interpolation between the key frames, benefiting from structural guidance provided by intermediate frames. The training of MaskINT incorporates masked token modeling. 
Our comprehensive set of experiments illustrates the efficacy and efficiency of MaskINT when compared to other diffusion-based methodologies. This research offers a practical solution for text-based video editing and showcases the potential of non-autoregressive masked generative transformers in this domain.
\end{abstract}




==> sec2/1_intro.tex <==
% \section{Introduction}
% \label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}





==> sec2/2_formatting.tex <==
% \section{Formatting your paper}
% \label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.




% \vspace{-0.5em}
\section{Related Work}
% \vspace{-0.5em}
\subsection{Diffusion Models}
% \vspace{-0.5em}
\paragraph{Diffusion Models in Image Editing. }
Leveraging the advancements of Stable Diffusion (SD) \citep{rombach2022high}, numerous studies have achieved significant success in the field of text-based image editing \citep{zhang2023adding, mou2023t2i,tumanyan2023plug,kawar2023imagic,hertz2022prompt,zhang2023sine,parmar2023zero, meng2021sdedit, couairon2022diffedit}. 
For example, ControlNet \citep{zhang2023adding}, T2I-Adapter \citep{mou2023t2i}, and Composer \citep{huang2023composer} introduce spatial condition such as depth maps and edge maps, enabling text-to-image synthesis with the same structure as the input image.  
% 
The PNP \citep{tumanyan2023plug} incorporates DDIM inversion features \citep{song2020denoising} from the input image into the text-to-image generation process alongside SD, enabling image editing without the necessity of additional training or fine-tuning. 
Instructpix2pix \citep{brooks2023instructpix2pix} trains a conditional diffusion model for text-guided image editing using synthetic paired examples, which avoid the tedious inversion. 
Nevertheless, employing these methods on each video frame independently often leads to inconsistencies and flickering. 


\vspace{-0.5em}
\paragraph{Diffusion Models in Video Editing. }
Recently, difusion models also dominate the field of video generation and video editing \citep{singer2022make,ho2022imagen}. 
For example, Gen-1 \citep{esser2023structure} trains a video diffusion models on paired text-video datasets to generate videos with both depth map and text conditions. 
Meanwhile, several works utilize pre-trained image diffusion models to achieve video editing in a training-free way \citep{wu2022tune,yang2023rerender,qi2023fatezero,khachatryan2023text2video,zhang2023controlvideo,wang2023videocomposer}. To enable a cohesive global appearance among edited frames, a common approach in these studies involves extending the attention module of SD to encompass multiple frames and conducting cross-frame attention. 
For example, Tune-A-Video \citep{wu2022tune} fine-tunes SD to a single video to perform video editing. 
Text2video-zero \citep{khachatryan2023text2video} performs cross-frame attention of each frame on the first frame to preserve appearance consistency. 
ControlVideo \citep{zhang2023controlvideo} extends ControlNet with fully cross-frame attention to joint edit all frames and further improves the performance with interleaved-frame smoother. 
TokenFlow \citep{geyer2023tokenflow} enhance PNP \citep{tumanyan2023plug} with extended-attention to jointly edit a few key frames at each denoising step and propagate them throughout the video based on nearest-neighbor field. 
% 
On the contrary, our work only utilize existing image diffusion models to edit two key frames, rather than all video frames. 
% Similarly, TokenFlow \citep{geyer2023tokenflow} jointly edits a few key frames by leveraging the PNP enhanced with extended attention. These edited frames are then propagated throughout the video using a nearest-neighbor field, relying on the inter-frame correspondences of DDIM-inverted features. 



% MagicEdit
% MagicProp

\vspace{-0.5em}
\subsection{Generative Transformers}
\vspace{-0.5em}

% Transformers have been widely used in both image and video generation. 
Following GPT \citep{brown2020language}, many pioneer works \citep{esser2021taming, yu2022vectorquantized,le2021ccvs, ge2022long,hong2022cogvideo} transfer images and videos into discrete tokens with VQGAN \citep{esser2021taming}, and perform image/video generation in an autoregressive way, where tokens are generated sequentially based on previous output. 
Nevertheless, these autoregressive methods become exceedingly time-consuming when the length of the token sequence increases.
% 
In recent times, non-autoregressive generative transformers, capable of simultaneously generating all tokens in parallel, have emerged as efficient solutions for image and video generation \citep{chang2022maskgit,yu2023magvit}. 
Specifically, MaskGiT \citep{chang2022maskgit} first shows the capability and efficiency  of non-autoregressive transformers in image generation. It can be seamlessly extended to tasks like inpainting and extrapolation by applying various initial mask constraints. 
MUSE \citep{chang2023muse} achieves state-of-the-art performance in text-to-image generation by training on large-scale text-image datasets and brings significantly efficiency improvement. 
% Moreover, MUSE can perform mask-free local editing by iteratively masking and resampling a random subset of tokens while being guided by text prompts. 
StyleDrop \citep{sohn2023styledrop} further finetunes Muse with human feedback to perform text-to-image generation guided with a reference style image. 
To control spatial layout, MaskSketch \citep{bashkirova2023masksketch} proposes a sampling strategy based on the similarity of attention maps to introduce structural guidance into MaskGiT. Nevertheless, this implicit structure condition is suboptimal. 
% 


In the filed of video generation, 
MaskViT \citep{gupta2023maskvit} employ 2D tokenizer and trains a bidirectional window transformer to perform frame prediction. 
Phenaki \citep{villegas2023phenaki} trains a masked transformer to generate short video clips condition on text prompt and extends it to arbitrary long video generation with different prompts in an autoregressive way. 
MAGVIT \citep{yu2023magvit} utilizes 3D  tokenizer to quantize a video into spatial-temporal visual tokens and trains a single model to perform multiple video editing tasks. 
However, to the best of our knowledge, there is currently no existing literature in the field of video editing utilizing masked generative transformers. Besides, there is a notable absence of research that delves into explicit structural control within masked generative transformers.






\vspace{-0.5em}
\section{Preliminaries}
\vspace{-0.5em}
\subsection{Masked Generative Transformers}
\vspace{-0.5em}
Masked generative transformers \citep{chang2022maskgit} follow a two-stage pipeline. In the first stage, an image is quantized into a sequence of discrete tokens via a Vector-Quantized (VQ) auto-encoder \citep{esser2021taming}. 
In detail, given an image $\textbf{I} \in \mathbb{R}^{H \times W \times 3}$, an encoder $\mathcal{E}$ encodes it into a series of latent vectors and discretize them through a nearest neighbour look up in a codebook of quantized embeddings with size $M$. 
To this end, an image can be represented with a sequence of codebook's indices $\mathbf{Z} = [z_i]_{i=1}^{h \times w}, z_i \in \{1,2,...,M\}$, where $h$ and $w$ is the resolution of latent features. A decoder $\mathcal{D}$ can reconstruct the indices back to image $\mathcal{D}(\mathbf{Z}) \approx \mathbf{I}$. 
% 
% 
In the second stage, a bidirectional transformer model \cite{vaswani2017attention} is learned with Masked Token Modeling (MTM). 
Specifically, during training, a random mask ratio $r \in (0,1)$ is selected and $[\gamma(r) \cdot h \times w]$ tokens in $Z$ are replaced with a special $\texttt{[MASK]}$ token, where $\gamma(r)$ is a mask scheduling function \citep{chang2022maskgit}. We denote the corrupted sequence with masked tokens as $\mathbf{\Bar{Z}}$ and conditions such as class labels or text description as $\mathbf{c}$. 
Given the training dataset $\mathbb{D}$, a BERT \citep{devlin2018bert} parameterized by $\Phi$ is learned to minimize the cross-entropy loss between the predicted and the ground truth token at each masked position: 
\begin{equation}
    \mathcal{L}_{MTM} = \mathop{\mathbb{E}}_{\mathbf{Z} \in \mathbb{D} } \left[ \sum_{ \Bar{z_i}= \texttt{[MASK]} }  -\log p_{\Phi}(z_i | \mathbf{\Bar{Z}}, \mathbf{c}) \right]
\end{equation}

During inference time, non-autoregressive decoding is applied to generate images. In detail, given the conditions $\mathbf{c}$, all tokens are initialized as \texttt{[MASK]} tokens. At step $k$, all tokens are predicted in parallel while only tokens with the highest prediction scores are kept. The remaining tokens with least prediction scores are masked out and repredicted in the next iteration. The mask ratio at each step is determined by $\gamma(\frac{k}{K})$, where $K$ is the total number of iteration steps. 



\vspace{-0.5em}
\subsection{ControlNet}
\vspace{-0.5em}
\paragraph{Latent Diffusion Models} 
% Denoising Diffusion Probabilistic Models (DDPM) \citep{ho2020denoising} generate images by progressively removing noise from an initial Gaussian noisy image in $T$ time steps. 
Denoising Diffusion Probabilistic Models (DDPM) \citep{ho2020denoising} generate images through a progressive noise removal process applied to an initial Gaussian noisy image, carried out over a span of $T$ time steps.
To enable efficient on high-resolution image generation, Latent Diffusion models \citep{rombach2022high} (a.k.a. Stable Diffusion) operates the diffusion process in the latent space of an autoencoder. First, an encoder $\mathcal{E}$ compresses an image $\mathbf{I}$ to a low-resolution latent code $x=\mathcal{E}(\mathbf{I}) \in \mathbb{R}^{h \times w \times c}$. Second, a U-Net $\epsilon_\theta$ with attention modules \citep{vaswani2017attention} is trained to remove the noise with loss function: 
\begin{equation}
    \mathcal{L}_{LDM} =  \mathbb{E}_{x_0, \epsilon \sim N(0, I), t\sim  } \| \epsilon - \epsilon_\theta (x_t, t, \tau) \|_2^2, 
\end{equation}
where $\tau$ is the text prompt and $x_t$ is the noisy latent sample at timestep $t$. 
Stable Diffusion is trained on datasets with billion scale text-image pairs, which serves as the foundation model of many generation tasks. 


\paragraph{ControlNet} 
In practice, it's challenging to design accurate text prompt to generate desired image. Furthermore, ControlNet \citep{zhang2023adding}  is proposed to provide spatial layout conditions such as edge map, depth map, and human poses. In detail, ControlNet train the same U-Net architecture as SD and finetune it with specific conditions. We denote ControlNet as $\epsilon_\theta(x_t, t, \tau, s)$, where $s$ is the spatial layout condition. 



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{framework.pdf}
    \caption{Overview of MaskINT. MaskINT disentangle the video editing task into two separate stages, i.e., key frame joint editing and structure-aware frame interpolation. }
    \label{fig:framework}
\end{figure}

\vspace{-0.5em}
\section{Methodology}

\vspace{-0.5em}
\subsection{Overview}
\vspace{-0.5em}
Figure \ref{fig:framework} shows an overview of our framework. 
We disentangle the video editing task into key frame joint editing stage and structure-aware frame interpolation stage. 
% 
Specifically, given a video clip with $N$ frames $ \{\mathbf{I}^i\}_{i=1}^N$, 
in the first stage, with the input text prompt $\mathbf{\tau}$, we simultaneously edit two key frames, i.e., the initial frame $\mathbf{I}^1$ and last frame $\mathbf{I}^N$, using existing image-editing model $g(\cdot)$ (i.e., ControlNet \citep{zhang2023adding} ) that requires no additional tuning.  
% This process results in the creation of 
This frame based joint editing module provides high-quality coherent edited frames $\mathbf{^*I}^1, \mathbf{^*I}^N = g(\mathbf{I}^1, \mathbf{I}^N, \mathbf{\tau})$ and is highly efficient on a pair of frame.
% 
% 
In the second stage, MaskINT performs structure-aware frame interpolation via non-autoregressive transformers. The entire edited video frames are generated by $\{ \mathbf{^*I}^i \}_{i=1}^{N} = f_\Phi(\mathbf{^*I}^1, \mathbf{^*I}^N,  \{ \mathbf{S}^i\}_{i=1}^N )$,  where $\mathbf{S}^i \in [0,1]^{H\times W \times 1}$ is the structural condition (i.e., the HED edge map\citep{xie2015holistically}).   
% 
% 
Our MaskINT is trained with masked token modeling (MTM) on video only datasets, conditioning on the structural signal $ \{ \mathbf{S}^i\}_{i=1}^N $ as well as two key frames (i.e., the initial frame $\mathbf{I}^1$ and last frame $\mathbf{I}^N$). 




% 


\vspace{-0.5em}
\subsection{Key frames Joint Editing}
\vspace{-0.5em}

To maintain the structure layout of selected key frames, we utilize ControlNet \citep{zhang2023adding} to edit $\mathbf{I}^1$ and $\mathbf{I}^N$ based on text prompt $\tau$ as well as their edge maps $\mathbf{S}^1$ and $\mathbf{S}^N$. 
However, even with the identical noise, applying ControlNet to each key frames individually, i.e., $\eps_\theta(x_t^1, t, \tau, \mathbf{S}^1)$ and $\eps_\theta(x_t^N, t, \tau, \mathbf{S}^N)$,  cannot guarantee the appearance consistency. 

To address this issue, following previous work \citep{wu2022tune, geyer2023tokenflow, zhang2023controlvideo}, we extend the self-attention blocks to simultaneously process multiple key frames. 
In the original U-Net of SD, the self-attention block projects the noisy feature map $x_t^j$ of $j^{th}$ frame at time step $t$ into query $\mathbf{Q}^j$, key $\mathbf{K}^j$, value  $\mathbf{V}^j$. 
We extend the self-attention blocks to perform attention across all selected key frames by concatenating their keys and values and calculate the attention by 
\begin{equation}
    \label{eq:joint_attn}
    \text{JointAttn}(\mathbf{Q}^j, \{ \mathbf{K}^j \}_{j \in \{1,N\}}, \{ \mathbf{V}^j \}_{j \in \{1,N\}} ) = \text{Softmax}(\dfrac{ \mathbf{Q}^j [\mathbf{K}^1, \mathbf{K}^N ]^\mathbf{T} }{ \sqrt{c} } ) [\mathbf{V}^1, \mathbf{V}^N]
\end{equation}

Note that although only two frames were used in Eq.\ref{eq:joint_attn}, this joint editing can seamlessly generalize to any number of key frames, at the cost of long processing time and  
huge demand in resources.


\vspace{-0.5em}
\subsection{MaskINT}

\vspace{-0.5em}

\paragraph{Structure-aware Window-Restricted Transformer. }
Previous masked generative transformers \citep{chang2022maskgit,yu2023magvit} employ a pure transformer with global attention \citep{vaswani2017attention}. 
However, this architecture lacks the control of structure in generation, and it is computationally extensive when applied to videos. Thus, we propose the structure-aware window-restricted transformer, a simple yet effective method to integrating structure conditions into video generation. 
% 
% 
% 
Specifically, we tokenize both RGB frames and edge maps with an off-the-shelf 2D VQ tokenizer \citep{esser2021taming}. 
We utilize 2D VQ rather than 3D VQ \citep{yu2023magvit} to accommodate varying numbers of frames and frame rate without constraints. 
We denote the tokens from RGB frames as $\mathbf{^cZ} = \{ ^cz_i\}_{i=1}^{N \times h \times w}$ (color token) and tokens from edge maps as $\mathbf{^sZ}=\{ ^sz_i\}_{i=1}^{N \times h \times w}$ (structure token), where $^sz_i$, $^cz_i \in \{1,2,...,M\}$, where $M$ is the codebook size.  
% 
Subsequently, two distinct embedding layers $e^C(\cdot)$ and $e^S(\cdot)$ are learned to map token indices $\mathbf{^cZ}$ and $\mathbf{^sZ}$ into their respective embedding spaces. Learnable 2D spatial positional encoding $\mathbf{P^S}$ and temporal positional encoding $\mathbf{P^T}$ are also added \citep{bertasius2021space}. Thus, the input can be formulated by $\mathbf{X} = e^c(\mathbf{^cZ}) + e^s(\mathbf{^sZ}) + \mathbf{P^S} + \mathbf{P^T} \in \mathbb{R}^{N \times h \times w \times c}$. 
Empirical results indicate that this straightforward addition operation of two types of embedding is remarkably effective to control the structure in generated frames. 
% 
% 
% 
Moreover, given that there is no substantial motion between consecutive frames, we adopt self-attention within a restricted window to further mitigate computational overhead, following MaskViT \citep{gupta2023maskvit}. 
In detail, our approach involves two distinct stages of attention. Initially, we employ spatial window attention, confining attention to tokens within a frame of dimensions $1 \times h \times w$. Subsequently, we extend this to spatial-temporal window attention, which confines attention to tokens within a tube of dimensions $N \times h_w \times w_w$, where $h_w$ and $w_w$ is the window size, where $h_w << h$ and $w_w << w$, which greatly reduce the complexity.
% 
Besides, to further reduce computation of transformer, we also add a shallow convolution layers to downsample $\mathbf{X}$ before the transformer encoder layers and an upsample layer at the end. 

\vspace{-0.5em}
\paragraph{Training. }
By fully disentangling  key frames editing and frame interpolation into distinct stages, our model no longer necessitates paired videos for training. Consequently, we can train MaskINT using video only datasets.
% 
% 
% 
Denote the color token of $i^{th}$ RGB frame as $\mathbf{^cZ}^i=\{^cz^i\}_{i=1}^{h\times w}$. 
During the training time, we keep color tokens of the initial frame $\mathbf{^cZ}^1$ and last frame $\mathbf{^cZ}^N$, and randomly replace $[\gamma(r) \cdot (N-2)\cdot N] $  color tokens of intermediate frames with the \texttt{[MASK]} tokens. We denote this corrupted video color tokens as $\mathbf{\Bar{^cZ}} = \{ \mathbf{^cZ}^1, \mathbf{\Bar{^cZ}}^2, ..., \mathbf{\Bar{^cZ}}^{N-1}, \mathbf{^cZ}^N \}$. 
The structure-aware window-restricted transformer with parameters $\Theta$ is trained by 

\begin{equation}
    \mathcal{L}_{MTM} = \mathop{\mathbb{E}}_{\mathbf{^cZ}, \mathbf{^sZ} \in 
\mathbb{D} } \left[ \sum_{ \Bar{^cz_i}= \texttt{[MASK]} }  -\log p_{\Theta}(z_i | \mathbf{\Bar{^cZ}}, \mathbf{^sZ}) \right]
\end{equation}
To avoid overfitting the structural condition, we random dropout a few structural tokens and replace them with zero embeddings during the training time. 


\vspace{-0.5em} 
\paragraph{Inference. }
During the inference time, our MaskINT can seamlessly generalize to perform frame interpolation between the jointly edited frames, although it is only trained with regular videos. 
% although never trained on paired data
Specifically, we tokenize the the initial and last edited frames $\mathbf{^*I}^1$ and $\mathbf{^*I}^N$ from Stage 1 into color tokens $\mathbf{^{c}_*Z}^1$ and $\mathbf{^{c}_*Z}^N$, and initialize color tokens of all intermediate frames $\{ \mathbf{\Bar{^cZ}}^2, ..., \mathbf{\Bar{^cZ}}^{N-1} \}$ with \texttt{[MASK]} tokens. 
We follow the iterative decoding in MaskGiT \citep{chang2022maskgit} with a total number of $K$ steps. At step $k$, we predict all color tokens in parallel and keep tokens with the highest confidence score. 



\vspace{-0.5em}
\section{Experiments}
\vspace{-0.5em}

\subsection{Settings}
\vspace{-0.5em}
\paragraph{Implementation Details. }
We train our model with $100k$ videos from ShutterStock website\footnote{\href{https://www.shutterstock.com/video}{https://www.shutterstock.com/video}}. During training time, we random select a $T=16$ video clip with frame interval $1,2,4$ from each video and resize it to $384\times 672$. We utilize Retina-VQ \citep{dubeyretinavq} with $8$ downsample ratio, i.e., each frame has $48\times84$ tokens. 
We employ Transformer-Base as our MaskINT and optimized it from scratch with the AdamW optimizer \cite{loshchilov2018decoupled} for a duration of $100$ epochs. The initial learning rate is set to $1e-4$ and decayed with cosine schedule. 
During the inference time, we set the number of decoding step $K$ to $32$ and the temperature $t$ to $4.5$.  

\vspace{-0.5em} 
\paragraph{Evaluation. } %
Following \citep{wu2022tune}, we use the $40$ object-centric videos of the DAVIS dataset \citep{Pont-Tuset_arXiv_2017}, covering humans, animals, vehicles, etc. 
Besides, we also select $30$ videos from the ShutterStock dataset. For each video, we manually design 5 edited prompts, including object editing, background changes and style transfers. 
Regarding the comparison methods, we select methods that built upon text-to-image diffusion models, including  TokenFlow \citep{geyer2023tokenflow}, Text-to-video zero \citep{khachatryan2023text2video}, and ControlVideo \citep{zhang2023controlvideo}. We also consider apply ControlNet to each frame individually  with the same initial noise as baseline. 

\vspace{-0.5em} 
\paragraph{Metrics. } %
Following previous works \citep{zhang2023controlvideo,qi2023fatezero}, we assess the quality of the generated videos using CLIP \citep{radford2021learning}. 
In detail, we evaluate 1) temporal consistency (in short, Tem-Con), which calculates the average cosine similarity of all pairs of consecutive frames. 2) prompt consistency (in short, Tem-Con), which calculates the average cosine similarity between given text prompt and all video frames. 
To evaluate the efficiency, we report the duration required for generating a 16-frame video clip on a single NVIDIA A6000 GPU. 



\vspace{-0.5em} 
\subsection{Results}
\vspace{-0.5em} 


\begin{table}[!ht]
    \caption{\small{Quantitative comparisons on the quality of the generated videos. ``Tem-Con" stands for temporal consistency, and ``Pro-Con" stands for prompt consistency.} }
    \label{tab:comparison}
    
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|cc|cc|c}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{DAVIS} & \multicolumn{2}{c|}{ShutterStock} & \multirow{2}{*}{Time} \\
         & Tem-Con & Pro-Con &  Tem-Con & Pro-Con &  \\
        \midrule 
        ControlNet per frame \citep{zhang2023adding} & 0.9137 &  0.3136 & 0.9419 & 0.3040 & 50s \\

        Text2Video-zero \citep{khachatryan2023text2video} & 0.9642 & 0.3124 & 0.9811 & 0.3036 & 60s \\
        TokenFlow \citep{geyer2023tokenflow} & 0.9774 & 0.3169 & 0.9869 & 0.3133 &  150s \\
        ControlVideo-edge \citep{zhang2023controlvideo} & 0.9746 & 0.3143 & 0.9864 & 0.3032 & 120s \\
        MaskINT (ours) & 0.9519 & 0.3112 & 0.9714 & 0.3038 & 22s \\
    \bottomrule
    \end{tabular}
    }

\end{table}


\vspace{-0.5em}
\paragraph{Quantitative Comparisons. }
Table \ref{tab:comparison} summarize the performance of these methods on both DAVIS and ShutterStock datasets. 
Notably, our method achieves comparable performance with diffusion methods, in terms of both temporal consistency and prompt consistency, while brings a significant acceleration in processing speed. In detail, MaskINT is almost 5.5 times faster than ControlVideo \citep{zhang2023controlvideo}, whose fully cross-frame attention is computationally extensive. Moreover, MaskINT is nearly 7 times faster than TokenFlow \citep{geyer2023tokenflow}, whose DDIM inversion is time-consuming. 
On the contrary, our acceleration is derived from a combination of a relatively lightweight network design and a reduced number of decoding steps in masked generative transformers. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{examples2.pdf}
    \caption{ \small{Examples of video editing with MaskINT. Frames with red bounding box are jointly edited key frames. We mask out human faces in input video for privacy protection.} }
    \label{fig:example}
\end{figure}


\vspace{-0.5em}
\paragraph{Qualitative Comparisons. } 

Fig. \ref{fig:teaser}(a) and Fig. \ref{fig:example} show samples of the edited videos with MaskINT. 
Our methods excel in producing temporally consistent videos that faithfully adhere to the provided text prompts. This extends to a wide range of applications, encompassing tasks such as stylization, background editing, foreground editing, and more. It also works well on challenging videos with substantial motion, such as dancing and running. 
% Note that, our MaskINT is only trained with realistic videos, but it can still generalize to all kinds of stylized videos.  
% 
Moreover, Fig. \ref{fig:cmp} provides a qualitative comparison of MaskINT to other baselines. 
Remarkably, diffusion methods \citep{geyer2023tokenflow,khachatryan2023text2video,zhang2023controlvideo} can ensure the consistency of overall appearance, but sometimes cannot maintain the consistency of detailed regions. For example, both TokenFlow \citep{geyer2023tokenflow} and Text2Video-Zero\citep{khachatryan2023text2video} exhibit noticeable artifacts in the leg region of the human subjects. ControlVideo \citep{zhang2023controlvideo} produces inconsistent hats. The potential explanation lies in the fact that these methods offer control over temporal consistency implicitly. 
Our MaskINT consistently interpolates the intermediate frames based on the structure condition and even maintain better consistency in local regions. 




\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{cmp.pdf}
    \caption{ \small{Qualitative comparisons with diffusion-based methods. More examples are shown in Appendix. } }
    \label{fig:cmp}
\end{figure}



\vspace{-0.5em}
\subsection{Ablation Studies}
\vspace{-0.5em}
\paragraph{Number of of key frames}
Although our model is trained with frame interpolation by default, MaskINT can seamlessly generalize to an arbitrary number of key frames. 
In this ablation study, we assess the impact of varying the quantity of key frames on performance on ShutterStock dataset.
As shown in the left part of Table \ref{tab:ablation}, with an increase in the number of key frames, the model exhibits a marginal improvement in performance. Generally, with more information, performing frame interpolation is easier. 
However, simultaneously editing more key frames requires longer time due to the global attention among them. 



\begin{table}[!ht]

    \caption{ \small{Ablation study on ShutterStock dataset of the number of key frames and the number of decoding steps $K$. ``Tem-Con" stands for temporal consistency and ``Pro-Con" stands for prompt consistency.} }
    \label{tab:ablation}

    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
    % \caption{\small{Ablation study on the number of key frames}}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|c|c}
        \toprule
        \# key frames  & Tem-Con & Pro-Con &  Time \\
        \midrule
        2 & 0.9714 & 0.3038 & 22s \\
        % 2 & 1, 8 & 0.9698 & \\
        3 &  0.9721 & 0.3051 & 26s \\ 
        4 &  0.9728 & 0.3069 & 29s \\
    \bottomrule
    \end{tabular}
    }  
    % \caption{ {Ablation study of the number of key frames.} }
    \end{minipage}
    % 
    % 
    % 
    \begin{minipage}{0.48\textwidth}
    
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|c|c}
        \toprule
        decoding step $K$  & Tem-Con & Pro-Con &  Time \\
        \midrule
        % 2 & 1, 8 & 0.9698 & \\
        16 & 0.9691 & 0.3038 & 15s \\
        32 & 0.9714 & 0.3038 & 22s \\
        64 &  0.9719 & 0.3040 & 33s \\
    \bottomrule
    \end{tabular}
    }  
    % \caption{ {Ablation study of the number of decoding steps $K$.} }
    \end{minipage}
    
    

\end{table}


\vspace{-0.5em}
\paragraph{Decoding steps}
We also explore the number of decoding steps of the masked generative transformers in the second stage. 
The right part of Table \ref{tab:ablation} shows that more decoding steps can bring slight improvement on the temporal consistency, but requires more time. Considering the trade-off between performance and efficiency, we chose $K=32$ steps by default in all experiments. 


\vspace{-0.5em}
\paragraph{key frames editing}
We can also employ other controls to edit key frames in the first stage due to the disentanglement. In this study, we utilize ControlNet with depth map to perform key frame editing, and still use MaskINT trained with HED edge conditions. 
In this configuration, we achieve a "Tem-Con" score of $0.9713$ and a "Pro-Con" score of $0.3159$ on ShutterStock, a result that closely aligns with the performance of joint editing using HED edges. 
Fig. \ref{fig:depth} shows an example of this setting. Editing key frames with depths provides more freedom over HED edge, but our method can still guarantee the consistency. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{depth.pdf}
    \caption{ \small{Examples of generated video from depth-based key frame editing. } }
    \label{fig:depth}
\end{figure}



\vspace{-0.5em}
\section{Limitation and Future Work}
\vspace{-0.5em}
One potential limitation of our approach is that it still necessitates the use of diffusion-based methods for key frame editing in the initial stage, which can still be somewhat time-consuming.
As for the future work,given that our approach disentangles video editing into two distinct stages, we intend to explore the integration of token-based methods, like Muse \citep{chang2023muse}, for image editing. This endeavor aims to further enhance the efficiency of the initial stage.


\vspace{-0.5em}
\section{Conclusion}
\vspace{-0.5em}
In this paper, we propose MaskINT towards consistent and efficient video editing with text prompt. 
MaskINT disentangle this task into key frames joint editing with diffusion methods and structure-aware frame interpolation with non-autoregressive masked transformers. 
Quantitative and qualitative experiments demonstrate that MaskINT achieves comparable performance with pure diffusion-based methods while significantly reduce the inference time. We are confident that our work demonstrates the substantial promise of non-autoregressive generative transformers within the realm of video editing.





==> sec2/3_finalcopy.tex <==
% \section{Final copy}

% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.




